Robot Fleet Learning via Policy Merging

Fleets of robots ingest massive amounts of heterogeneous streaming data silos generated by interacting with their environments, far more than what can be stored or transmitted with ease. At the same time, teams of robots should co-acquire diverse skills through their heterogeneous experiences in varied settings. How can we enable such fleet-level learning without having to transmit or centralize fleet-scale data? In this paper, we investigate policy merging (PoMe) from such distributed heterogeneous datasets as a potential solution. To efficiently merge policies in the fleet setting, we propose FLEET-MERGE, an instantiation of distributed learning that accounts for the permutation invariance that arises when parameterizing the control policies with recurrent neural networks. We show that FLEET-MERGE consolidates the behavior of policies trained on 50 tasks in the Meta-World environment, with good performance on nearly all training tasks at test time. Moreover, we introduce a novel robotic tool-use benchmark, FLEET-TOOLS, for fleet policy learning in compositional and contact-rich robot manipulation tasks, to validate the efficacy of FLEET-MERGE on the benchmark.

==> body/experiments.tex <==

\section{Experiments: Linear Policy Merging} 
\label{exp:linear_merging} 




 
In this setting, we use the optimal LQG controller to generate 
expert trajectories for multiple tasks. Similar to \cite{zhang2022multi}, our system has state dimension $n=4$ and control dimension $m=2$, and each task shares the same system matrix and only differs in the task matrix $Q=\alpha^{(h)} I_4$ where $h$ is in the set of $-2$ to $2$ in logspace. Following \cite{zhang2022multi}, we obtain a high dimensional observation by $y_t=Cx_t$ where $C \in \mathbb{R}^{50\times 4}$ is fixed and its entries are uniformly and independently sampled from a Gaussian distribution, which makes the matrix invertible with high probability. We train the controller parameter with the following procedure:
\begin{equation}
z_{t+1}=A_{\theta}  z_t+B_{\theta}  y_{t},\qquad 
{u}_t=C_{\theta}  z_t, \qquad
L=\sum_t^T \norm{\hat{u}_t-{u}_t}^2.
\end{equation}
Following \cite{zhang2022multi}, we then use the closed-loop rollout metric $\mathcal{T}(\pi)=\frac{1}{N} \sum_{i=1}^N \max_{t\le T} \norm{y^{i}_t-\hat{y}_t}^2$ to evaluate the learner's performance with respect to the expert, where $\hat{u}, \hat{y}$ denotes the input and output of the learner.

 We aim to learn a single set of $(A_{\theta}, B_{\theta}, C_{\theta})$ for the joint data distributions with policy merging, which does not require sharing the data across individual policy training. Therefore, the merged policy can be either a single-task policy or a multi-task policy (with different matrices $Q$). The environment dynamics $(A,B)$ are fixed. We then compare different kinds of merging algorithms by evaluating the performance of the merged policy. 
 
In Figure \ref{fig:linear_result} Left, we first observe that for the case with static feedback policies, simply \textit{average} $\pi(y)=K_\theta y$ can improve the performance over \textit{single-dataset} or \textit{single-task} that just use local data and even match policies that trained with shared data (\textit{multitask}) or task-specific data (\textit{task-specific}). We then compare the case with dynamic policies (Figure \ref{fig:linear_result} Right) and note that the \textit{gradient-based} method can outperform the \textit{alternation-based} method that searches in only the space of permutation matrices. These two methods also outperform the naive averaging method (\textit{average}) which does not consider basin ambiguity and\textit{single-task} which only trains with local dataset.



 
 \begin{figure*}[!t]
\centering 
\includegraphics[width=0.95\textwidth]{images/drake_benchmark.pdf}
\caption{Drake Tool-Use Benchmark. We develop several tool-use tasks that focus on contact-rich motions and compositions, including using spatula, knife, hammer, and  wrench in the Drake \cite{drake} simulator. }
\label{fig:drake_benchmark}
\end{figure*}
 \begin{figure*}[!t]
\centering 
\includegraphics[width=1\textwidth]{images/drake_merging_results_new.pdf}
\caption{{\textbf{(Top)} Mode Connectivity Setting.} Recall the performance barrier, and the x-axis denotes the interpolation ratios $\lambda$ between the two models and the y-axis represents the success rates of the policy rollouts. {\textbf{(Left)}  Skill Merging Setting.} The x-axis denotes the non-IIDness (increasing to the right). The performance is upper-bounded and lower-bounded by joint training and single-shot merging. {\textbf{(Right)} Decentralized Policy Learning Setting.} The x-axis denotes the training epochs between every time we merge the model  (decreasing to the right).}
\label{fig:mode_connectivity} 
\end{figure*}





 




\section{Experiments: Nonlinear Policy Merging}
\label{exp:multitask_task}





\subsection{Drake Tool-use Tasks}

In this section, we develop a new robot learning environment in Drake \cite{drake},  with different tool-use tasks, to evaluate the performance of our policy merging algorithms. Tool-use tasks require policy learning that can tackle diverse data distributions,  as well as the compositional nature of robot tasks such as the affordance of the tools. We use the segmented tool and object point cloud as the agent observation, and the 6-dof translation and rotation as the agent action. The initial end-effector poses, the initial object pose, and the tool-in-hand poses are randomized at each episode. The task is determined successful when certain thresholds are met: for example, the pin is hammered down in the hammering task.   We use different tool-object pairs as different tasks 
for tool-use. We have considered mostly 4 task families (wrench, hammer, spatula, and knife), and for each task family, we find 3D models for tool and object from Mcmaster Carr Catalog and datasets such as Shapenet \citep{chang2015shapenet}. See Appendix \ref{appendix:drake} for more details on the descriptions of the task, dataset, and the scripted expert. The policy network architecture is a very standard PointNet \citep{qi2017pointnet} (Max pooling after a few MLPs).  

We first trained multiple feedforward policies for a single task and single datasets with imitation learning, and then evaluate the performance barrier for every pair of the trained policies. We observe that with an algorithm to find the permutation alignment, we can achieve almost zero performance barriers. We also apply the decentralized policy learning framework in the tool-use benchmarks. We show that we can acquire a policy by merging the policies trained on each dataset, without sharing data or changing the input-output behavior of each individual model. Furthermore, in the decentralized learning setting, the merged policy is robust against the number of models and the number of times that models are merged.




\subsection{Meta-world}

In this section, we experiment with imitation learning on the popular Meta-world benchmark \cite{yu2020meta}, which has 50 distinct manipulation tasks. We use frozen ResNet features on the images as policy inputs. In Figure \ref{fig:mode_connectivity}, we compare different merging algorithms to measure the mode connectivity and observed that there are almost no performance barriers between the policies. We show similar observations across different architectures, different inputs and metrics, and large-scale settings in the Appendix \ref{appendix:metaworld}. Moreover, we compared the merged policy with different non-IIDness and observe that the gradient-based algorithms achieve the best performance. 




Additionally, we consider multi-task policy learning settings with decentralized training. In Figure \ref{fig:metaworld_dec}, the alternation-based merging algorithm can outperform naive averaging across different levels of communication efficiency and participation ratios.  We also demonstrate that a simple multi-task learning agent can solve all 50 tasks in the benchmark jointly without pooling data together but achieve similar performance.  We also conduct ablation studies of our algorithm in supervised learning settings in the appendix section \ref{appendix:ablation}.



  \begin{figure*}[!t]
\centering 
\includegraphics[width=1\textwidth]{images/mode_connectivity.pdf}
\caption{\textbf{(Left)} Mode Connectivity for Policies on Meta-World. We observe that the connectivity curve is basically flat. \textbf{(Right)} Different Algorithms Applied on Merging Policies from Multiple Tasks.}
\label{fig:drake_results} 
\end{figure*}


 \begin{figure*}[!t]
\centering 
\includegraphics[width=1\textwidth]{images/metaworld_fedavg_epoch_results.pdf}
\caption{We showed that FedAvg with our merged algorithm achieves better performance on Metaworld in decentralized settings, when changing the communication epochs (10 tasks) and the partial participation ratios (25 tasks). The performance is upper-bounded and lower-bounded by the joint policy success rates and the merged policy that averages only once.}
\label{fig:metaworld_results}
\end{figure*}


==> body/method.tex <==

\section{Linear Policy Merging} 


\begin{figure*}[!t]
\centering 
\includegraphics[width=0.9\textwidth]{images/rnn_symmetry2.pdf}
\caption{A diagram for the permutation symmetries appeared in recurrent neural nets. The RNN permutation is motivated by the well-known invariance of controller performance under similarity transformations in LQG control. In addition to the challenge of merging multiple layers jointly, we note two additional challenges: merging multiple models rather than two models and merging in the time horizon. }
\label{fig:rnn}
\end{figure*}

We start by considering merging the policies in the linear control case. As mentioned above, the linear dynamic parameterization is invariant up to similarity transformation. 




\subsection{Invariance of LQG to Coordinate Transformation}

 In view of the LQG ambiguity, recent works \cite{zheng2021analysis} have provided algorithms and results as follows: there exists some invertible matrix $P$, such that the parameters   $(A_{\theta},B_{\theta},C_{\theta})$ of the dynamical  policy can be identified as $(A_{\hat{\theta}},B_{\hat{\theta}},C_{\hat{\theta}})$, satisfying 
\#\label{equ:exist_results}
\max\big\{\|A_{\hat{\theta}}-P^{-1}A_{\theta}P\|,~\|B_{\hat{\theta}}-P^{-1}B_{\theta}\|,~\|C_{\hat{\theta}}-C_{\theta}P\|\big\}\leq \epsilon,
\# 
with finite input-output sample guarantees. 



 
In   LQG problems, the policies can be viewed as dynamical systems parameterized by some matrices  $(A_{\theta} \in \mathbb{R}^{n\times n},B_{\theta}\in \mathbb{R}^{n\times d},C_{\theta}\in \mathbb{R}^{m\times n})$ where $n, m$ are the dimensions of observation and controls, and $d$ is the dimension of the latent state. In particular,  for each dataset $i\in[N]$. consider  the following dynamical policy:
\$
\label{linear_learner}
z_{t}=A_{\theta,i} z_{t-1}+B_{\theta,i} y_{t},\qquad 
u_t=C_{\theta,i} z_t,
\$
where we note that if it exactly recovers the optimal LQG controller, we will have the correspondences that $A_{\theta^*}=A+BK^*-L^*C$, $B_{\theta^*}=L^*$, and $C_{\theta^*}=K^*$. As shown in Algorithm \ref{alg:lqg_learner}, we train these controllers' parameters with gradient descent by  minimizing the sum of total $\mathcal{L}_2$ squared loss on the predicted action and the ground truth action from the LQG expert, that generates the trajectories 
${D}=\{\{(y_t^i,u_t^i)\}_{t=0,...T-1}\}_{i=1,..,M}$. 


Similar to the discussion above, these $\{A_{\theta,i},B_{\theta,i},C_{\theta,i}\}_{i\in[N]}$ can be close up to similarity transformation, if they are learned either from different datasets (for example decentralized/federated learning), or even different runs/initializations  of the same dataset (for example \cite{zheng2021analysis} when policy gradient methods are used), or just different factorization of the same learned Markov parameter (for example \cite{oymak2019non,tsiamis2019finite}). 


 





\subsection{Algorithm}
We propose two different types of merging algorithms to combine the policies. Both algorithms leverage iterative alternations to update each model's transform matrix and the merged parameters separately, in order to avoid the problem of bilinearity. The first algorithm leverages the closed-form solutions such as linear sum assignments, whereas the second algorithm  is based on gradient updates.

\subsubsection{Alternation Algorithm for finding permutations}

Our first approach is to focus on finding $N$ \textit{permutations} that merge the $N$ models, rather than allowing arbitrary invertible transformations. This type of approach turns out to generalize to the nonlinear problem setting, in section [TODO]. We define an objective to minimize the sum of distances of each individual model $\theta_i=\{A_{\theta,i},B_{\theta,i},C_{\theta,i}\}$ to the merged model $\bar{\theta}=\{A_{\bar{\theta}},B_{\bar{\theta}},C_{\bar{\theta}}\}$ through permutations $P_i$: 
\begin{equation}
\label{eq:linear_obj}
    \min_{\bar{\theta},\{P_i\}_{i=1}^N}\quad  g\left(\bar{\theta}, \{P_i\}\right) := \sum_{i=1}^N \norm{{A}_{\bar{\theta}} - P_i^\top A_{\theta,i}P_i}^2_F  + \norm{{B}_{\bar{\theta}} - P_i^\top B_{\theta,i}}^2_F  + \norm{{C}_{\bar{\theta}} - C_{\theta,i}P_i }^2_F.
\end{equation}
 
We use alternations to make the bilinearity problem in Eq. \eqref{eq:linear_obj} tractable. We separate each iteration into two steps. In the centering step, we fix $P_i$ and optimize for $\bar{\theta}$. This is equivalent to computing the mean of all individual transformed $\theta_i$ to estimate the merged model $\bar{\theta}$.
 

\begin{align*}
&\arg\min_{\bar{\theta}} ~\ g\left(\bar{\theta}; \{P_i\}\right) = \left\{\bar{A}, \bar{B}, \bar{C}\right\}, \text{ where} \\
\bar{A}=\frac{1}{N}\sum\limits_{i=1}^N &A_{\theta,i}^{\top}P_i A_{\theta,i}, \; \bar{B}=\frac{1}{N}\sum\limits_{i=1}^N  P_i^\top B_{\theta,i}, \; \bar{C}=\frac{1}{N}\sum\limits_{i=1}^N C_{\theta,i}P_i. 
\end{align*}


In the transform step, for each agent $i$, we fix the $A_i$ and $\bar{A}$, and we compute the permutation matrix $P_i$ by solving a linear sum assignment problem to align the local model with the merged model. To avoid the two-sided linear sum assignment problem, we reuse the permutation matrix from the previous iteration $P_i'$ (where $P_0=I$) for the current iteration, and then we can solve it as a regular linear sum assignment \cite{bertsekas1998network}. 

\begin{align}
& \min\limits_{P_i \in \mathcal{P}} \norm{{A}_{\bar{\theta}} - P_i^\top A_{\theta,i}P_i}^2_F  + \norm{{B}_{\bar{\theta}} - P_i^\top B_{\theta,i} }^2_F  + \norm{{C}_{\bar{\theta}} - C_{\theta,i}P_i }^2_F 
\end{align}
which can be simplified to
\begin{align}\max_{P_i\in \Pi}~~~ \langle P_i,  A_{\theta,i}^{\top}P_i' {A}_{\bar{\theta}}    +     B_{\theta,i}{B}_{\bar{\theta}}^{\top } + C_{\theta,i}^{\top}{C}_{\bar{\theta}}   \rangle 
\end{align}

We note that there are a finite number ($N^2$ pair) of $(P,P')$ and the objective $\langle P_i, {\theta_1}P_{i-1}{\theta_2}^\top  \rangle$ is non-decreasing. Therefore this procedure is guaranteed to converge.  

\subsubsection{Joint Gradient-Based Algorithm for finding permutations}
 Our second approach for merging policies is to find a solution in the set of invertible matrices through gradient descent on equation \ref{eq:linear_obj}. Specifically, after rewriting the formulation, we can see that the problem is convex in each $P_i$ and ${A}_{\bar{\theta}},{B}_{\bar{\theta}},{C}_{\bar{\theta}}$ if we fix $\bar{\theta}$ or fix $P_i$ separately. Therefore for $N
$ models, we run alternating gradient descent to update those parameters to update the averaged model parameters $\bar{\theta}$ and $P$ (stack of $P_i$ separately).
 
 
 


\subsection{Analysis for Linear Dynamic Output Feedback Policy}
\label{analysis}
\label{dynamic_output_policy}
\lirui{on-going.} See appendix \ref{linear_analysis} for more detailed discussions on when merging can work for single-task and when it can work for multitask. We also present counter-examples.

\section{Nonlinear Policy Merging}

\subsection{RNN Permutation Symmetry}

 
We now look to generalize the analysis from the previous section to deep recurrent neural networks (RNNs), which are often used to implement \textit{nonlinear} dynamic policies.
Recurrent policies have achieved significant successes in robot policy learning, partly because real world robotics problems tend to be partially observable and require policies to have memory over past observations~\cite{bakker2001reinforcement}. Previous works on permutation symmetries in neural networks mostly focus on supervised learning problems with feedforward networks \cite{tatro2020optimizing,entezari2021role,ainsworth2022git,pena2022re}, with relatively little emphasis on recurrent architectures.   



In a deep Elman RNN~\citep{elman1990finding} with nonlinear activation function  $\sigma(\cdot)$, at each layer $l$ and timestep $t$ we recursively compute activations $h^{l}_t$ by:
\begin{equation}
    h^{l}_t = \sigma(W^{l}_{ih}h^{l-1}_t + W^{l}_{hh} h^l_{t-1} + b^l_h)
\end{equation}
where we define $h^0_t = x_t$ to be the input at each timestep and $h^l_0$ to be the initial RNN latent activations for each layer.

Note that a simple extension of the permutation symmetry for a feedforward network would fail in the RNN case. Consider a two-layer RNN without biases unrolled for two timesteps (see the appendix for the general case). Its outputs $(h^2_0, h^2_1)$ are unchanged if we modify the RNN with any permutation matrix $P$ as follows:
\begin{align}
  h_0^1&=\sigma(PW^1_{ih}x_0+PW^{1}_{hh}{P^\top}\cdot 0); h_0^2=\sigma(W^2_{ih}P^\top h_0^1+ W^{2}_{hh} \cdot 0) \\
  h_1^1&=\sigma(PW^1_{ih}x_1+PW^{1}_{hh}P^\top \cdot h_0^1); h_1^2=\sigma(W^2_{ih}P^\top h_1 ^1+ W^{2}_{hh} \cdot  h_0^2).
\end{align} 

 
Figure~\ref{fig:rnn} shows that by unrolling the RNN computation graph over multiple timesteps, the latent activations can be permuted independently at each timestep.
 However, since RNN parameters are shared over time, we can only apply a single permutation at each layer across all timesteps, i.e.,  $P_{i,0}=P_{i,1}=...=P_{i,T}$.  Hence we can simplify the permutation symmetry for RNNs from 
\begin{align}
     &h_t^{j}  =\sigma(P_{j,t} W^j_{ih} P_{j-1,t}^\top x_t+ {P_{j,t}} W^{j}_{hh} P_{j,t-1}^\top  \cdot h^{j}_{t-1} +P_{j,t}b^j_{ih}+P_{j,t}b^j_{hh}) %
\end{align}
to  
 \begin{align}
 &h_t^{j}  =\sigma(P_{j} W^j_{ih} P_{j-1}^\top x_t+ {P_{j}} W^{j}_{hh} P_{j}^\top  \cdot h^{j}_{t-1} +P_jb^j_{ih}+P_jb^j_{hh})
\end{align} 
where the permutation for latent weight  matrix applies for time symmetry (as in any state-space model), and the permutation for input weight matrix applies for layer symmetry. 
Our analysis of the RNN's permutation symmetries can also be extended to LSTMs and transformers~\cite{vaswani2017attention}.

In summary, an $L$-layer RNN with parameters:
\begin{equation}
   \theta = \{W^1_{ih},W^1_{hh},W^2_{ih},W^2_{hh},...,W^L_{ih},W^L_{hh}\},
\end{equation}
is invariant to permutations of its parameters of the form:
\begin{equation}
 \theta'=\{P_1W^1_{ih},P_1W^1_{hh},P_2W^2_{ih}P_1^\top ,P_2W^2_{hh}P_2^\top,...,W^L_{ih}P_L^\top,W^L_{hh}P_L^\top\},
\end{equation}
for any set of permutation matrices $(P_1, \cdots, P_L)$.


 \begin{figure*}[!t]
\centering 
\vspace{-10mm}
\includegraphics[width=1\textwidth]{images/linear_results.pdf}
\caption{Linear Single Task Results. \textbf{(Left)} We observe that even averaging linear policies can often improve performance to almost match joint training on the pooled data for single-task and match task-specific training for multi-task. \textbf{(Right)} We see that gradient-based methods to find general invertible matrix performs better than finding permutation matrix with alternations. }
\label{fig:linear_result}
\end{figure*}



\subsection{Alternation Algorithm for Finding Permutations}
We develop two different families of algorithms  to apply permutation matrices to merge many models: alternation-based algorithms and joint-training algorithms, in the same vein as the linear setting.
For alternation-based algorithms, our objective is to match the weights layer-by-layer between two different policies that can be recurrent or feedforward networks while keeping each separate network functionally equivalent. Specifically, we optimize the following objective: $   \min\limits_{\Pi_i} \sum\limits_{i=1}^N \norm{\text{vec}({\Pi_i(\theta))-\text{vec}(\bar{\theta}})}^2_F  
  $ to ensure the permuted parameter is close to the merged policy in Euclidean distance. Given any align functions $\textit{Align}(\bar{\theta},\theta)$, which can be Sinkhorn matching \cite{pena2022re}, optimal transport matching \cite{singh2020model}, or git-rebasin \cite{ainsworth2022git}, we can apply it to the inner loop of the alternation-based methods to find permutation.

\subsection{Data-based Algorithm of Merging $N$ Models}
Despite its simplicity, previous algorithms have assumed no data access for finding the permutations. If we are allowed to use data to find the permutations, then we can differentiate through the training objectives for optimization. We use the implicit-sinkhorn formulations \cite{mena2018learning,eisenberger2022unified}.  Specifically, we associate a set of permutation parameters $P_i$ for each weight  $\theta_i$, and we form the averaged model as $\bar{\theta
}=\frac{1}{K}\sum_{k=1}^K \theta_k$. We then jointly train to update the ``soft'' permutation matrices $P_k$ with the available trajectory data $D_{\text{perm}}=\{(y,u)\}$ with loss $L$ through the implicit Sinkhorn operators \cite{pena2022re}. The Sinkhorn operator  \cite{mena2018learning,eisenberger2022unified} is defined as a soft version of the linear sum assignment problem that is differentiable to allow flexible objectives:
\begin{equation}
S_\tau(X)=\argmax(\langle P,X\rangle_F+ \tau h(P))
\end{equation}
where $\tau$ is a hyperparameter that weights the strengths of the entropy regularization term $h(P)$, and $X$ is a soft version of the hard permutation matrix $P$. The reparametrization of the neural networks for one layer can be rewritten as 
\begin{equation}
     h_t^{j}=\sigma(S_\tau(P_{j,t}) W^j_{ih} S_\tau(P_{j-1,t})^\top x_t+ S_\tau({P_{j,t}}) W^{j}_{hh} S_\tau(P_{j,t-1})^\top  \cdot h^{j}_{t-1} +S_\tau(P_{j,t})b^j_{ih}+S_\tau(P_{j,t})b^j_{hh})
\end{equation} 

We find the flexible objective and the joint optimization of all layers of permutation matrices to be favorable. Specifically, at each training epoch, we compute the average of the merged model using the hard permutation matrix. We can then randomly interpolate between the merged model and each individual model, and minimize the training losses with respect to the permutation matrix associated with that interpolated model. Note that training the permutation parameters can be viewed as a \texttt{FedAvg} operation \cite{mcmahan2017communication} in federated learning and it does not require using data from one dataset for other models.

\begin{algorithm}
\label{alg:nonlinear_gradient}
\caption{Fed-Rebasin}
\begin{algorithmic}[1] 
\STATE \textbf{Input}:~~Local iteration number $E$,  step size $\gamma$, $N$ 
 model parameters $\theta_1,...,\theta_N$, $N$ permutation parameters $\mathcal{P}_1,...,\mathcal{P}_N$, $\mathcal{D}_{\text{perm},i}$ datasets used for finding permutations for model $i$.
  
\STATE{Initialize {individual models} $\theta_1,...,\theta_N$}
\FOR{{$t=0,...,E-1$}}
\STATE{\text{Average models:}~~$\bar\theta \gets \frac{1}{N}\sum_i \mathcal{P}_{i,hard}(\theta_i)$} \\
\FOR{{$i=0,...,N-1$}}
\STATE{\text{Sample data pair:}~~$(y,u)\sim D_{\text{perm},i}$}\\
\STATE{\text{Randomly sample $\epsilon$ from $(0,1)$}} \\
\STATE{\text{Interpolate model:}~~ $\Tilde{\theta}=\epsilon \theta_i +(1-\epsilon) \bar{\theta}$} \\
\STATE{\text{Compute loss:}~~ $\ell_i \gets L_{\Tilde \theta}(y,u)$}
\STATE{\text{Update soft $\mathcal{P}_i$:}~~$\mathcal{P}_i\gets \mathcal{P}_i-\gamma \nabla_{\mathcal{P}_i} \ell_i $}
\ENDFOR
\ENDFOR
\STATE{\text{Apply strict permutation $\mathcal{P}_{\text{hard}}$  on each model:}~~$\theta_i \gets \mathcal{P}_{\text{hard}}(\theta_i)$} \\
\STATE{\text{Average models:}~~$\bar\theta \gets \frac{1}{N}\sum_i \theta_i$}
\STATE {\bf Return}:~~$\bar\theta$
\end{algorithmic}
\end{algorithm}

\subsection{Policy Merging with Non-IID Datasets}

In practice, users can define how frequently the policies are merged and how many models are merged each time, under different Non-IID data distribution settings. We consider a setting where we are allowed to merge multiple times during training, which is analogous to the federated and decentralized settings.  We  could control different levels of non-IIDness by training each dataset's underlying distribution as a ``class''  and sampling from a Dirichlet distribution to form a mixed dataset.  To further study this setting, we use other two commonly used metrics in decentralized learning  -- the number of local updates epochs, and the participation ratio of data sources.  In addition to the naive aggregation function in the {\texttt{FedAvg}}  algorithm, we can use the algorithm proposed in the previous sections to try to merge multiple models. This can be seen as we train the model, we also add merging with other models to our objective. When learning from diverse datasets, the source of non-IIDness can come from different experts, different sensors, or even different tasks.  

 

==> body/problem.tex <==

\section{Preliminaries and Problem Setup}
\label{problem}



\paragraph{Mode connectivity. } DO we need this?




\subsection{Invariance under Transformations and Mode Connectivity}

\subsection{Rebasin}

The policy 
may be invariant to certain transformations of the parameter and preserves the input-output behavior, when parameterized by (feedforward) neural networks or linear dynamical systems. 



\paragraph{Permutation invariance under NN parameterization.} 
Under neural network parameterization, similar invariance behavior of the parameterized policy also occurs, under the {\it permutation transformation}  \cite{ainsworth2022git}. Specifically, consider an $L$-layer feedforward neural network  to parameterize a static-feedback policy. At the $l$-th layer, the feedforward parameterization gives $
z_{l+1}  =\sigma(W_l z_l + b_l),$ 
where $z_l$ and $z_{l+1}$ correspond to the input and output, and $W_l,b_l$ are the weight and bias,  of layer $l$, respectively. We use $\theta=\{W_0,W_1,\cdots,W_{L-1}\}$ to denote the set of parameters in this case. Note that $z_0=o_t$ is the input, i.e., the observation, and $z_{L}=u_t$ is the output, i.e., the control action, of the policy. Under permutation transformation, we have a new formula 
\$
z_{l+1}  =\sigma(P_{l+1} W_l P_{l}^\top z_l + P_{l+1}b_l),
\$
where $\mathcal{P}=\{P_l\}_{l=0}^L$ denotes a set of permutation matrices for each layer $l$. This permutation transformation does not change the input-output relationship from $o_t$ to $u_t$. We let $\theta'=\{P_0W_0,P_1W_1P_0,...,W_{L-1}P_{L-1}\}$. Note that compared to the linear control case, the invariance transformation is restricted to permutation matrices instead of general invertible matrices, due to the possible nonlinearity of the activation functions. 


 
\paragraph{Similarity invariance under linear dynamic parameterization.}
For linear control problems, the policies are parameterized  by linear dynamical systems, with parameter 
$\theta:=(A_{\theta},B_{\theta},C_{\theta})$ (c.f. Eq. \eqref{equ:dynamic_policy_para_general}). It is known that such a parameterization is invariant  under the {\it similarity transformation} of the parameters: 
\begin{align}
z_{t}&=PA_{\theta}{P^{-1}}\cdot z_{t-1}+PB_{\theta}y_{t}\\
u_t&=C_{\theta} P^{-1} z_t 
\end{align}
where we use $(z_t)$ to denote the state estimate $\hat{x}_t$ in Eq. \eqref{equ:dynamic_policy_para_general}, and $P$ can be any invertible matrix.  
Note that the recursive formula here allows the control action $u_t$  to be dependent on the history $h_t:=(u_{0:t-1},y_{0:t-1},y_t)$.  Note that the input-output behavior of the system \eqref{equ:system} is {\it preserved} under similarity transformation of the state-space representations, i.e., under the new system $(A_{\theta'},B_{\theta'},C_{\theta'})$ where $A_{\theta'}=P^{-1}A_{\theta}P$, $B_{\theta'}=P^{-1} B_{\theta}$, and $C_{\theta'}=C_{\theta} P$, and by changing the covariance matrix $\Sigma_W$ to $\Sigma_W':=P \Sigma_W P^{-1}$. 

\paragraph{Mode connectivity.}
To quantify the degree of invariance under different transformations, we also introduce the notion of {\it loss barrier}, inspired by the definition in the supervised learning setting for studying the  {\it mode connectivity} of neural networks \cite{frankle2020linear,ainsworth2022git}\kz{maybe more refs}. 
Specifically, given two sets of parameters $\theta,\theta'$ such that $\mathcal{L}(\theta)\approx \mathcal{L}(\theta')$,   the \textit{imitation loss barrier} of the policies is defined as $\max_{\lambda\in [0,1]} \mathcal{L}((1-\lambda)\theta+\lambda \theta')-\frac{1}{2}(\mathcal{L}(\theta)+\mathcal{L}(\theta'))$. {A smaller loss barrier generally implies a flatter landscape between $\theta$ and $\theta'$.}  Moreover, we can also extend the definition to measuring task performance in the context of imitation learning. Given task performance metric $\mathcal{T}$ (which could be the success rates of completing certain tasks, or the cumulative rewards), the {\it task performance barrier} is defined as  $\max_{\lambda\in [0,1]} \frac{1}{2}(\mathcal{T}(\theta_A)+\mathcal{T}(\theta_B))-\mathcal{T}((1-\lambda)\theta_A+\lambda \theta_B)$, where the sign is flipped to model the rewards achieved in accomplishing certain tasks. 



\subsection{Policy Merging} 
Consider the setting where there are $N$ datasets $D_1,\cdots,D_N$, where each dataset $D_i$ contains the rollout trajectory data by deploying different behavior policies, on the same dynamics. We use $\mathcal{D}_1,\cdots,\mathcal{D}_N$ to denote the corresponding probability distributions that generate the datasets. To exploit multi-task robotic data to train a general policy, we aim to minimize the  objective: 
\begin{equation}
    \min_{\theta}~~\sum_{i\in[N]}\frac{|D_i|}{|D|}\cL_i(\theta)
\end{equation}   where $\cL_i(\theta)$ is the imitation learning loss on dataset $\mathcal{D}_i$. The simplest way to solve the problem is to jointly pool all the data together for training. We consider the policy merging problem in this work, which tries to learn a general policy for multiple data distributions by sharing network weights instead of sharing data. Sharing the weights, as a compression of data, is more communication efficient and yet more challenging. The key challenge of this problem is how to do model aggregation that takes in a set of policy models and outputs a merged policy for the joint data distribution. 



\paragraph{Example:  Federated/Decentralized  learning.} 

In practice, we are not limited to merging only once after training, the training process with merging weights remains communication-efficient without sharing data, which is analogous to the decentralized or federated learning settings.  For instance, {\texttt{FedAvg}}   \citep{mcmahan2017communication} is one algorithm that optimizes this objective by with model-sharing among data sources multiple times during training. 

\subsection{Permutation Invariances}

\section{Problem (Old)}
\subsection{Problem Setup}



We consider the general setting of controller/policy design when the system state may not be  observed. We also refer to this case as   control with \emph{partial observations} or \emph{output feedback}. Let 
$\mathcal{S}$, $\mathcal{A}$, and $\mathcal{O}$ represent the spaces of state, action, and observation, respectively. In general, let $\pi: (\mathcal{O}\times \mathcal{A})^{\NN}\times \cO  \to \mathcal{A}$   be a (deterministic) policy which maps the history of observation and actions until the current timestep  to the next action. In particular, at timestep $t\geq 0$, let $H_t:=(o_0,a_0,\cdots,a_{t-1},o_t)$ denote the history until time $t$, then $a_t=\pi(h_t)$. In the special case where only the \emph{current}  observation $o_t$ is used,  we have $\pi:\cO\to \cA$ and choose $a_t=\pi(o_t)$. This is also referred to as \emph{static output feedback} in controls  literature. Finally, for the special case with fully observability, $o_t=s_t$ and it usually does not lose optimality to consider state-feedback policies $\pi:\cS\to\cA$ and choose $a_t=\pi(s_t)$. 
To respect the notational convention in (deep) reinforcement learning and control, we will oftentimes use the notation of $(o,a,s)$ in the    RL setting with general (and nonlinear) dynamics and observation channels, and  $(y,u,x)$ when it comes to  the classical linear control setting, to denote observation, control action, and state, respectively.  One special case of the  classical control settings  is the linear quadratic Gaussian  (LQG) problem stated below. \kz{propagate to appendix.}



\paragraph{Control with (possibly) partial observations.} We consider the general setting of controller/policy design when the system state may not be  observed. We also refer to this case as   control with \emph{partial observations} or \emph{output feedback}. Let 
$\mathcal{S}$, $\mathcal{A}$, and $\mathcal{O}$ represent the spaces of state, action, and observation, respectively. In general, let $\pi: (\mathcal{O}\times \mathcal{A})^{\NN}\times \cO  \to \mathcal{A}$   be a (deterministic) policy which maps the history of observation and actions until the current timestep  to the next action. In particular, at timestep $t\geq 0$, let $h_t:=(o_0,a_0,\cdots,a_{t-1},o_t)$ denote the history until time $t$, then $a_t=\pi(h_t)$. In the special case where only the \emph{current}  observation $o_t$ is used,  we have $\pi:\cO\to \cA$ and choose $a_t=\pi(o_t)$. This is also referred to as \emph{static output feedback} in controls  literature. Finally, for the special case with fully observability, $o_t=s_t$ and it usually does not lose optimality to consider state-feedback policies $\pi:\cS\to\cA$ and choose $a_t=\pi(s_t)$. 
To respect the notational convention in (deep) reinforcement learning and control, we will oftentimes use the notation of $(o,a,s)$ in the    RL setting with general (and nonlinear) dynamics and observation channels, and  $(y,u,x)$ when it comes to  the classical linear control setting, to denote observation, control action, and state, respectively.  One special case of the  classical control settings  is the linear quadratic Gaussian  (LQG) problem stated below. \kz{propagate to appendix.}

\textbf{Linear quadratic control.} Consider an  LQG problem, with linear time-invariant (LTI) dynamic system characterized by $(A \in \mathbb{R}^{n_x \times n_x},B \in \mathbb{R}^{n_x \times m},C\in \mathbb{R}^{n \times n_x})$. The system evolves as  follows:
\#\label{equ:system}
x_{t+1}=Ax_t+Bu_t+w_t,\qquad \qquad 
y_t=Cx_t+v_t\notag
\# 
for $t\geq 0$, $x_t$ and $u_t$ denote the state and action, respectively, and $w_t,v_t$ are both i.i.d. Gaussian noises drawn from $\cN(0,\Sigma_W)$ and $\cN(0,\Sigma_V)$ with covariance matrices $\Sigma_W,\Sigma_V$. The initial state $x_0$ is also drawn from a  Gaussian distribution $\cN(0,\Sigma_0)$. Consider the stage-cost function $c(x,u):=x^\top Qx+u^\top R u$ for some positive semidefinite $Q$ and positive definite $R$.  It is known that under standard controllability and observability assumptions, the optimal solution  can be attained by some \emph{dynamic}  policy. Specifically, the optimal control $u^*_t$ is determined as $u^*_t=K^*\hat{x}_t$ for some feedback gain matrix $K^*\in \RR^{m\times n_x}$, where $\hat{x}_t$ is the estimation of the underlying state $x_t$ using the history until $t$, and can be obtained in a recursive way using Kalman filter separately. It is referred to as a \emph{dynamic} policy as the composition of Kalman filtering and linear feedback control yields a dynamical system, with $y_t$ being the input, $\hat{x}_t$ being the state, and $u_t$ being the output. Such a linear system can also be viewed as a one-layer and linear recurrent neural network that recursively encodes the history of observations to control actions. See \S\ref{sec:add_background} for more details about the background on LQG. 

\subsection{Behavior Cloning}
 As one of the most widely used imitation learning approaches, behavior cloning \cite{osa2018algorithmic,bagnell2015invitation} aims to   learn a policy $\pi_\theta:(\mathcal{O}\times \mathcal{A})^{\NN}\times \cO  \to \mathcal{A}$, parameterized by some parameter $\theta\in \RR^d$,   that in general maps the histories to actions, by imitating some expert policy $\pi^*:(\mathcal{O}\times \mathcal{A})^{\NN}\times \cO  \to \mathcal{A}$.  Let 
 ${D}=\{\{(y_t^i,u_t^i)\}_{t=0,...T-1}\}_{i=1,..,M}$ denote  the $M$ rollout trajectories generated under expert policy $\pi^*$, and $\cD$ denote the corresponding distribution (of the trajectories) that generate $D$. In the ``visuomotor'' policy learning  setting we may conduct experiments later, the observation $y_t$ is usually high-dimensional images. The objective in behavior cloning is 
  usually defined as 
$\ell({\theta})= \sum_{i\in[M],t\in([T]-1)}\norm{\pi_\theta(h_t^i)-u_t^i}^2$, where $h_t^i:=(y_0^i,u_0^i,\cdots,u_{t-1}^i,y_t^i)$ denotes the history in trajectory $i$ until timestep $t$. In the special case with  full observability and static feedback, the objective can be  simplified as  $\ell({\theta})= \sum_{i\in[M],t\in([T]-1)}\norm{\pi_\theta(s_t^i)-u_t^i}^2$, where $s_t^i=o_t^i$ is the observed state at timestep $t$ in trajectory $i$. 


\subsection{Invariance under Transformations and Mode Connectivity}

The policy 
may be invariant to certain transformations of the parameter and preserves the input-output behavior, when parameterized by (feedforward) neural networks or linear dynamical systems. 



\paragraph{Permutation invariance under NN parameterization.} 
Under neural network parameterization, similar invariance behavior of the parameterized policy also occurs, under the {\it permutation transformation}  \cite{ainsworth2022git}. Specifically, consider an $L$-layer feedforward neural network  to parameterize a static-feedback policy. At the $l$-th layer, the feedforward parameterization gives $
z_{l+1}  =\sigma(W_l z_l + b_l),$ 
where $z_l$ and $z_{l+1}$ correspond to the input and output, and $W_l,b_l$ are the weight and bias,  of layer $l$, respectively. We use $\theta=\{W_0,W_1,\cdots,W_{L-1}\}$ to denote the set of parameters in this case. Note that $z_0=o_t$ is the input, i.e., the observation, and $z_{L}=u_t$ is the output, i.e., the control action, of the policy. Under permutation transformation, we have a new formula 
\$
z_{l+1}  =\sigma(P_{l+1} W_l P_{l}^\top z_l + P_{l+1}b_l),
\$
where $\mathcal{P}=\{P_l\}_{l=0}^L$ denotes a set of permutation matrices for each layer $l$. This permutation transformation does not change the input-output relationship from $o_t$ to $u_t$. We let $\theta'=\{P_0W_0,P_1W_1P_0,...,W_{L-1}P_{L-1}\}$. Note that compared to the linear control case, the invariance transformation is restricted to permutation matrices instead of general invertible matrices, due to the possible nonlinearity of the activation functions. 


 
\paragraph{Similarity invariance under linear dynamic parameterization.}
For linear control problems, the policies are parameterized  by linear dynamical systems, with parameter 
$\theta:=(A_{\theta},B_{\theta},C_{\theta})$ (c.f. Eq. \eqref{equ:dynamic_policy_para_general}). It is known that such a parameterization is invariant  under the {\it similarity transformation} of the parameters: 
\begin{align}
z_{t}&=PA_{\theta}{P^{-1}}\cdot z_{t-1}+PB_{\theta}y_{t}\\
u_t&=C_{\theta} P^{-1} z_t 
\end{align}
where we use $(z_t)$ to denote the state estimate $\hat{x}_t$ in Eq. \eqref{equ:dynamic_policy_para_general}, and $P$ can be any invertible matrix.  
Note that the recursive formula here allows the control action $u_t$  to be dependent on the history $h_t:=(u_{0:t-1},y_{0:t-1},y_t)$.  Note that the input-output behavior of the system \eqref{equ:system} is {\it preserved} under similarity transformation of the state-space representations, i.e., under the new system $(A_{\theta'},B_{\theta'},C_{\theta'})$ where $A_{\theta'}=P^{-1}A_{\theta}P$, $B_{\theta'}=P^{-1} B_{\theta}$, and $C_{\theta'}=C_{\theta} P$, and by changing the covariance matrix $\Sigma_W$ to $\Sigma_W':=P \Sigma_W P^{-1}$. 




\subsection{Policy Merging} 
Consider the setting where there are $N$ datasets $D_1,\cdots,D_N$, where each dataset $D_i$ contains the rollout trajectory data by deploying different behavior policies, on the same dynamics. We use $\mathcal{D}_1,\cdots,\mathcal{D}_N$ to denote the corresponding probability distributions that generate the datasets. To exploit multi-task robotic data to train a general policy, we aim to minimize the  objective: 
\begin{equation}
    \min_{\theta}~~\sum_{i\in[N]}\frac{|D_i|}{|D|}\cL_i(\theta)
\end{equation}   where $\cL_i(\theta)$ is the imitation learning loss on dataset $\mathcal{D}_i$. The simplest way to solve the problem is to jointly pool all the data together for training. We consider the policy merging problem in this work, which tries to learn a general policy for multiple data distributions by sharing network weights instead of sharing data. Sharing the weights, as a compression of data, is more communication efficient and yet more challenging. The key challenge of this problem is how to do model aggregation that takes in a set of policy models and outputs a merged policy for the joint data distribution. 



\paragraph{Example:  Federated/Decentralized  learning.} 

In practice, we are not limited to merging only once after training, the training process with merging weights remains communication-efficient without sharing data, which is analogous to the decentralized or federated learning settings.  For instance, {\texttt{FedAvg}}   \citep{mcmahan2017communication} is one algorithm that optimizes this objective by with model-sharing among data sources multiple times during training. 



The remaining sections of the paper are organized as follows: We first discuss the linear policy setting and algorithms for finding the similarity transformation to merge the models. We then discuss the general nonlinear imitation learning setting for visuomotor policy learning and discuss a permutation symmetry for RNNs, as well as algorithms to merge policies. We extend this single-shot policy merging setting to merging networks during training, which is a novel decentralized policy learning setting and achieves better performance in multitask learning. Finally, we instantiate these ideas with numerical experiments as well as experiments on robotic benchmarks.

==> preamble/characters.tex <==

% Special letters: blackboard, mathcal, widehat % djhsu magic
\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname bb#1\endcsname{\ensuremath{\mathbb{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname fr#1\endcsname{\ensuremath{\mathfrak{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop


\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname eul#1\endcsname{\ensuremath{\EuScript{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop


\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname scr#1\endcsname{\ensuremath{\mathscr{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop


\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname bhat#1\endcsname{\ensuremath{\hat{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname btil#1\endcsname{\ensuremath{\tilde{\mathbf{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname bst#1\endcsname{\ensuremath{\mathbf{#1}^\star}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname bst#1\endcsname{\ensuremath{\mathbf{#1}^\star}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname b#1\endcsname{\ensuremath{\mathbf{#1}}}}
\ddefloop abcdeghijklnopqrstuvwxyz\ddefloop

\def\ddefloop#1{\ifx\ddefloop#1\else\ddef{#1}\expandafter\ddefloop\fi}
\def\ddef#1{\expandafter\def\csname barb#1\endcsname{\ensuremath{\bar{\mathbf{#1}}}}}
\ddefloop abcdefghijklmnopqrstuvwxyz\ddefloop

\def\ddef#1{\expandafter\def\csname c#1\endcsname{\ensuremath{\mathcal{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname h#1\endcsname{\ensuremath{\widehat{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname hc#1\endcsname{\ensuremath{\widehat{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname t#1\endcsname{\ensuremath{\widetilde{#1}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop
\def\ddef#1{\expandafter\def\csname tc#1\endcsname{\ensuremath{\widetilde{\mathcal{#1}}}}}
\ddefloop ABCDEFGHIJKLMNOPQRSTUVWXYZ\ddefloop

==> preamble/math_commands.tex <==
%!TEX root = ../arxiv_main.tex

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
%\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
%\def\Algref#1{Algorithm~\ref{#1}}
%\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
%\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
 
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\newcommand{\lirui}[1]{\textcolor{blue}{[Lirui: #1]}}
\newcommand{\vect}[2]{\ensuremath{\begin{bmatrix} #1 & #2 \end{bmatrix}}}
\newcommand{\vectt}[2]{\ensuremath{\begin{bmatrix} #1 \\ #2 \end{bmatrix}}}
\renewcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}
\newcommand{\abs}[1]{\ensuremath{{\left\vert #1 \right\vert}}}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\kron}{\ensuremath{\otimes}}
\newcommand{\inprod}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\prox}{\ensuremath{\textbf{prox}}}
\newcommand{\Span}{\ensuremath{\textbf{span}}}

\newcommand{\paren}[1]{\mathopen{}\left(#1\right)\mathclose{}}
\newcommand{\curly}[1]{\mathopen{}\left\{#1\right\}\mathclose{}}
\newcommand{\brac}[1]{\mathopen{}\left[#1\right]\mathclose{}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\der}[2]{\frac{d\, #1}{d\, #2}}
\newcommand{\proj}{\operatorname{proj}}

\let\ab\allowbreak
\usepackage{amsmath, amsfonts, bm, amssymb}
% \usepackage{amsfonts, graphicx, grffile,fullpage, float, latexsym, mathtools}
\usepackage{latexsym, mathtools}
\usepackage{graphicx}
\usepackage{float}
\usepackage{ifthen}
% \usepackage{hyperref}
%\Crefname{Algorithm}{Algorithms}
% % \usepackage{algorithm}
% % \usepackage{algpseudocode}
% % \usepackage{wrapfig}
\usepackage{thmtools, thm-restate}
\usepackage{enumitem}
% % \usepackage[round]{natbib}
% % \renewcommand{\bibname}{References}
% % \renewcommand{\bibsection}{\subsubsection*{\bibname}}
% \usepackage[caption=false]{subfig}

\usepackage{calc}
\usepackage{tikz}


% ========== Custom operators and definitions ==========
% -- General --
\DeclareMathOperator{\bmtx}{\begin{bmatrix}}
\DeclareMathOperator{\emtx}{\end{bmatrix}}
\DeclareMathOperator{\T}{^\top}
\DeclareMathOperator{\I}{^{-1}}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\tr}{\mathrm{tr}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\sign}{sign}
\let\Re\relax
% \let \det \relax
% \DeclareMathOperator{\det}{\textbf{det}}
% \DeclareMathOperator{\Re}{\mathbb{R}e}
\DeclareMathOperator{\kernel}{Ker}
\DeclareMathOperator{\indeg}{deg_{in}}
\DeclareMathOperator{\outdeg}{deg_{out}}
\DeclareMathOperator{\degbar}{\overline{deg}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator{\subjectto}{subject\ to}
\DeclareMathOperator{\lmin}{\lambda_\textup{min}}
\DeclareMathOperator{\lmax}{\lambda_\textup{max}}
\DeclareMathOperator{\smin}{\sigma_\textup{min}}
\DeclareMathOperator{\smax}{\sigma_\textup{max}}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\blkdiag}{blkdiag}
%\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\epi}{\textbf{epi }}
\DeclareMathOperator{\cov}{\textbf{cov}}

%BEGIN SHORTHANDS
%-- Shorthands --
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}
\newcommand{\calVbar} {\ensuremath{\overline{\calV}}}
\newcommand{\asm}{\ensuremath{\alpha}-supermodular}
\newcommand{\Asm}{\ensuremath{\alpha}-Supermodular}
\DeclareMathOperator{\E}{\textbf{E}}
\let \P \relax
\DeclareMathOperator{\P}{\mathbb{P}}
\DeclareMathOperator{\var}{var}

\newcommand{\bzero}{\ensuremath{\bm{0}}}
\newcommand{\bone}{\ensuremath{\bm{1}}}
\newcommand{\bA}{\ensuremath{\bm{A}}}
\newcommand{\bB}{\ensuremath{\bm{B}}}
\newcommand{\bC}{\ensuremath{\bm{C}}}
\newcommand{\bD}{\ensuremath{\bm{D}}}
\newcommand{\bE}{\ensuremath{\bm{E}}}
\newcommand{\bF}{\ensuremath{\bm{F}}}
\newcommand{\bG}{\ensuremath{\bm{G}}}
\newcommand{\bH}{\ensuremath{\bm{H}}}
\newcommand{\bI}{\ensuremath{\bm{I}}}
\newcommand{\bJ}{\ensuremath{\bm{J}}}
\newcommand{\bK}{\ensuremath{\bm{K}}}
\newcommand{\bL}{\ensuremath{\bm{L}}}
\newcommand{\bM}{\ensuremath{\bm{M}}}
\newcommand{\bN}{\ensuremath{\bm{N}}}
\newcommand{\bO}{\ensuremath{\bm{O}}}
\newcommand{\bP}{\ensuremath{\bm{P}}}
\newcommand{\bQ}{\ensuremath{\bm{Q}}}
\newcommand{\bR}{\ensuremath{\bm{R}}}
\newcommand{\bS}{\ensuremath{\bm{S}}}
\newcommand{\bT}{\ensuremath{\bm{T}}}
\newcommand{\bU}{\ensuremath{\bm{U}}}
\newcommand{\bV}{\ensuremath{\bm{V}}}
\newcommand{\bW}{\ensuremath{\bm{W}}}
\newcommand{\bX}{\ensuremath{\bm{X}}}
\newcommand{\bY}{\ensuremath{\bm{Y}}}
\newcommand{\bZ}{\ensuremath{\bm{Z}}}
\newcommand{\ba}{\ensuremath{\bm{a}}}
\newcommand{\bb}{\ensuremath{\bm{b}}}
\newcommand{\bc}{\ensuremath{\bm{c}}}
\newcommand{\bd}{\ensuremath{\bm{d}}}
\newcommand{\be}{\ensuremath{\bm{e}}}
\newcommand{\bbf}{\ensuremath{\bm{f}}}
\newcommand{\bg}{\ensuremath{\bm{g}}}
\newcommand{\bh}{\ensuremath{\bm{h}}}
\newcommand{\bi}{\ensuremath{\bm{i}}}
\newcommand{\bj}{\ensuremath{\bm{j}}}
\newcommand{\bk}{\ensuremath{\bm{k}}}
\newcommand{\bl}{\ensuremath{\bm{l}}}
\newcommand{\bbm}{\ensuremath{\bm{m}}}
\newcommand{\bn}{\ensuremath{\bm{n}}}
\newcommand{\bo}{\ensuremath{\bm{o}}}
\newcommand{\bp}{\ensuremath{\bm{p}}}
\newcommand{\bq}{\ensuremath{\bm{q}}}
\newcommand{\br}{\ensuremath{\bm{r}}}
\newcommand{\bs}{\ensuremath{\bm{s}}}
\newcommand{\bt}{\ensuremath{\bm{t}}}
\newcommand{\bu}{\ensuremath{\bm{u}}}
\newcommand{\bv}{\ensuremath{\bm{v}}}
\newcommand{\bw}{\ensuremath{\bm{w}}}
\newcommand{\bx}{\ensuremath{\bm{x}}}
\newcommand{\by}{\ensuremath{\bm{y}}}
\newcommand{\bz}{\ensuremath{\bm{z}}}
\newcommand{\bPi}{\ensuremath{\bm{\Pi}}}
\newcommand{\bPhi}{\ensuremath{\bm{\Phi}}}
\newcommand{\bLambda}{\ensuremath{\bm{\Lambda}}}
\newcommand{\calSigma}{\ensuremath{\bm{\Sigma}}}
\newcommand{\bMt}{\ensuremath{\bm{{\tilde{M}}}}}
\newcommand{\bpi}{\ensuremath{\bm{\pi}}}
\newcommand{\balpha}{\ensuremath{\bm{\alpha}}}
\newcommand{\bbeta}{\ensuremath{\bm{\beta}}}
\newcommand{\bgamma}{\ensuremath{\bm{\gamma}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}

\newcommand{\hatL}{\ensuremath{\hat L}}
\newcommand{\bfA}{\ensuremath{\mathbf{A}}}
\newcommand{\bfB}{\ensuremath{\mathbf{B}}}
\newcommand{\bfC}{\ensuremath{\mathbf{C}}}
\newcommand{\bfD}{\ensuremath{\mathbf{D}}}
\newcommand{\bfE}{\ensuremath{\mathbf{E}}}
\newcommand{\bfF}{\ensuremath{\mathbf{F}}}
\newcommand{\bfG}{\ensuremath{\mathbf{G}}}
\newcommand{\bfH}{\ensuremath{\mathbf{H}}}
\newcommand{\bfI}{\ensuremath{\mathbf{I}}}
\newcommand{\bfJ}{\ensuremath{\mathbf{J}}}
\newcommand{\bfK}{\ensuremath{\mathbf{K}}}
\newcommand{\bfL}{\ensuremath{\mathbf{L}}}
\newcommand{\bfM}{\ensuremath{\mathbf{M}}}
\newcommand{\bfN}{\ensuremath{\mathbf{N}}}
\newcommand{\bfO}{\ensuremath{\mathbf{O}}}
\newcommand{\bfP}{\ensuremath{\mathbf{P}}}
\newcommand{\bfQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\bfR}{\ensuremath{\mathbf{R}}}
\newcommand{\bfS}{\ensuremath{\mathbf{S}}}
\newcommand{\bfT}{\ensuremath{\mathbf{T}}}
\newcommand{\bfU}{\ensuremath{\mathbf{U}}}
\newcommand{\bfV}{\ensuremath{\mathbf{V}}}
\newcommand{\bfW}{\ensuremath{\mathbf{W}}}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\bfa}{\ensuremath{\mathbf{a}}}
\newcommand{\bfb}{\ensuremath{\mathbf{b}}}
\newcommand{\bfc}{\ensuremath{\mathbf{c}}}
\newcommand{\bfd}{\ensuremath{\mathbf{d}}}
\newcommand{\bfe}{\ensuremath{\mathbf{e}}}
\newcommand{\bff}{\ensuremath{\mathbf{f}}}
\newcommand{\bfg}{\ensuremath{\mathbf{g}}}
\newcommand{\bfh}{\ensuremath{\mathbf{h}}}
\newcommand{\bfi}{\ensuremath{\mathbf{i}}}
\newcommand{\bfj}{\ensuremath{\mathbf{j}}}
\newcommand{\bfk}{\ensuremath{\mathbf{k}}}
\newcommand{\bfl}{\ensuremath{\mathbf{l}}}
\newcommand{\bfm}{\ensuremath{\mathbf{m}}}
\newcommand{\bfn}{\ensuremath{\mathbf{n}}}
\newcommand{\bfo}{\ensuremath{\mathbf{o}}}
\newcommand{\bfp}{\ensuremath{\mathbf{p}}}
\newcommand{\bfq}{\ensuremath{\mathbf{q}}}
\newcommand{\bfr}{\ensuremath{\mathbf{r}}}
\newcommand{\bfs}{\ensuremath{\mathbf{s}}}
\newcommand{\bft}{\ensuremath{\mathbf{t}}}
\newcommand{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand{\bfv}{\ensuremath{\mathbf{v}}}
\newcommand{\bfw}{\ensuremath{\mathbf{w}}}
\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
\newcommand{\measuredU}{\tilde u}

\newcommand{\Xdata}{\ensuremath{\mathbf{X}}}
\newcommand{\Vdata}{\ensuremath{\mathbf{U}}}
\newcommand{\Zdata}{\ensuremath{\mathbf{Z}}}
\newcommand{\Fdata}{\ensuremath{\mathbf{F}}}

%\def\st/{\textsuperscript{st}}
\def\nd/{\textsuperscript{nd}}
\def\rd/{\textsuperscript{rd}}
\def\th/{\textsuperscript{th}}

\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\del}{\ensuremath{\partial}}
\newcommand{\ones}{\ensuremath{\bm{1}}}
\newcommand{\zeros}{\ensuremath{\bm{0}}}
\newcommand{\MSE}{\ensuremath{\textup{MSE}}}
\newcommand{\bbb}{\ensuremath{\bm{{\bar{b}}}}}
\newcommand{\bxb}{\ensuremath{\bm{{\bar{x}}}}}
\newcommand{\bPb}{\ensuremath{\bm{{\bar{P}}}}}
\newcommand{\bPu}{\ensuremath{\bm{{\underaccent{\bar}{P}}}}}
\newcommand{\bbt}{\ensuremath{\bm{{\tilde{b}}}}}
\newcommand{\bPt}{\ensuremath{\bm{{\tilde{P}}}}}


%norms
\newcommand{\vect}[2]{\ensuremath{\begin{bmatrix} #1 & #2 \end{bmatrix}}}
\newcommand{\vectt}[2]{\ensuremath{\begin{bmatrix} #1 \\ #2 \end{bmatrix}}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}
\newcommand{\abs}[1]{\ensuremath{{\left\vert #1 \right\vert}}}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\kron}{\ensuremath{\otimes}}
\newcommand{\inprod}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\prox}{\ensuremath{\textbf{prox}}}
\newcommand{\Span}{\ensuremath{\textbf{span}}}

\newcommand{\paren}[1]{\mathopen{}\left(#1\right)\mathclose{}}
\newcommand{\curly}[1]{\mathopen{}\left\{#1\right\}\mathclose{}}
\newcommand{\brac}[1]{\mathopen{}\left[#1\right]\mathclose{}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\der}[2]{\frac{d\, #1}{d\, #2}}
\newcommand{\proj}{\operatorname{proj}}

% \newcommand{\qedhere}{\hfill\blacksquare}

\newcommand{\bmat}[1]{\begin{bmatrix} #1\end{bmatrix} }
\newcommand{\NC}{\operatorname{NC}}
\newcommand{\AC}{\operatorname{AC}}
\newcommand{\RC}{\operatorname{RC}}
\newcommand{\Ne}{\operatorname{NE}}
\newcommand{\Ae}{\operatorname{AE}}


%%%%% STATS/ML


\newcommand{\st}[1]{{\color{red}st: #1}}
 
\newcommand{\symlambmin}{\ensuremath{\lambda_{\min}}}
\newcommand{\symlambmax}{\ensuremath{\lambda_{\max}}}

\newcommand{\vecop}{\operatorname{Vec}}
\newcommand{\dare}{\textnormal{\texttt{DARE}}}
\newcommand{\dlyap}{\textnormal{\texttt{dlyap}}}
\newcommand{\fcl}[1]{f_{\mathsf{cl}}^{#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\black}[1]{{\color{black}#1}}
\newcommand{\ER}{\mathrm{ER}}
\newcommand\norm[1]{\lVert#1\rVert}
\newcommand{\rmd}{\mathrm{d}}

%END SHORTHANDS


